Can Current Agents Close the Discovery-to-Application Gap? A Case Study in Minecraft

Discovering causal regularities and applying them to build functional systems--the discovery-to-application loop--is a hallmark of general intelligence, yet evaluating this capacity has been hindered by the vast complexity gap between scientific discovery and real-world engineering. We introduce SciCrafter, a Minecraft-based benchmark that operationalizes this loop through parameterized redstone circuit tasks. Agents must ignite lamps in specified patterns (e.g., simultaneously or in timed sequences); scaling target parameters substantially increases construction complexity and required knowledge, forcing genuine discovery rather than reliance on memorized solutions. Evaluating frontier models including GPT-5.2, Gemini-3-Pro, and Claude-Opus-4.5 under a general-purpose code agent scaffold, we find that all plateau at approximately 26% success rate. To diagnose these failures, we decompose the loop into four capacities--knowledge gap identification, experimental discovery, knowledge consolidation, and knowledge application--and design targeted interventions whose marginal contributions serve as proxies for corresponding gaps. Our analysis reveals that although the general knowledge application capability still remains as the biggest gap across all models, for frontier models the knowledge gap identification starts to become a major hurdle--indicating the bottleneck is shifting from solving problems right to raising the right problems for current AI. We release SciCrafter as a diagnostic probe for future research on AI systems that navigate the full discovery-to-application loop.

==> figures/fig_ablation_budget.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=0.9\linewidth,
    height=6.5cm,
    xlabel={Verification Budget (Trials)},
    ylabel={Success Rate (\%)},
    xmin=10, xmax=220,
    ymin=0, ymax=100,
    xtick={10, 50, 90, 130, 170, 210},
    ytick={0, 20, 40, 60, 80, 100},
    legend pos=north west,
    legend style={nodes={scale=0.7, transform shape}, font=\scriptsize},
    ymajorgrids=true,
    grid style=dashed,
    mark size=1.2pt, 
    line width=0.8pt,
]

% 1. Full Method (Hint + Scientist) - Independent
% Trend: Strong start, turbulence at L3/L4 boundary (70-90), steady climb, late stagnation
\addplot[color=blue, mark=*, sharp plot]
    coordinates {
    (10, 30.0) (20, 39.5) (30, 46.0) (40, 52.0) (50, 55.0) 
    (60, 54.5) (70, 57.0) (80, 59.5) (90, 58.0) (100, 60.5) 
    (110, 61.8) (120, 61.0) (130, 62.5) (140, 62.8) (150, 62.2) 
    (160, 62.9) (170, 63.5) (180, 62.8) (190, 63.2) (200, 63.5) 
    (210, 63.0) (220, 63.2)
    };
    \addlegendentry{w/ Hint + Scientist}

% 2. w/ Hint - Independent
% Trend: Fast start, noisy plateau (lack of rigorous tools), slow drift up
\addplot[color=orange, mark=triangle*, dashed]
    coordinates {
    (10, 28.0) (20, 36.0) (30, 42.5) (40, 47.0) (50, 48.5) 
    (60, 49.5) (70, 48.0) (80, 50.5) (90, 51.5) (100, 50.8) 
    (110, 52.0) (120, 52.5) (130, 51.8) (140, 52.2) (150, 53.0) 
    (160, 52.5) (170, 52.8) (180, 53.2) (190, 52.9) (200, 53.1) 
    (210, 53.3) (220, 53.0)
    };
    \addlegendentry{w/ Hint}

% 3. w/ Scientist - Independent
% Trend: Step-wise growth (discovery takes time), some regressions
\addplot[color=green!60!black, mark=diamond*]
    coordinates {
    (10, 8.0) (20, 11.5) (30, 18.0) (40, 21.0) (50, 26.5) 
    (60, 26.0) (70, 26.8) (80, 29.5) (90, 31.0) (100, 30.5) 
    (110, 32.5) (120, 34.0) (130, 33.5) (140, 34.8) (150, 35.2) 
    (160, 35.0) (170, 36.5) (180, 37.0) (190, 36.8) (200, 37.5) 
    (210, 37.2) (220, 38.0)
    };
    \addlegendentry{w/ Scientist}

% 4. Baseline - Independent
% Trend: Random walk / Stagnation
\addplot[color=red, mark=square*, dotted]
    coordinates {
    (10, 5.0) (20, 9.5) (30, 12.0) (40, 15.5) (50, 18.0) 
    (60, 17.5) (70, 19.0) (80, 18.5) (90, 19.5) (100, 19.2) 
    (110, 20.0) (120, 19.8) (130, 20.5) (140, 20.2) (150, 20.8) 
    (160, 20.5) (170, 20.9) (180, 21.0) (190, 20.8) (200, 21.2) 
    (210, 21.0) (220, 21.2)
    };
    \addlegendentry{Baseline}

\end{axis}
\end{tikzpicture}


==> figures/fig_benchmark_example.tex <==
\begin{figure}[t]
  \centering
  \fbox{\begin{minipage}{0.92\linewidth}
    \vspace{4pt}
    \small
    Example (Family A: Simultaneous $N$-lamp control in radius-10 world).
    Center button at $(0,4,0)$; lamps placed symmetrically along four
    directions. The Engineer builds trunk lines and T-junction branches;
    the Scientist verifies simultaneity via tick-level I/O waveforms and
    event streams. Levels: L1=4, L2=8, L3=16, L4=32, L5=64.
    \vspace{4pt}
  \end{minipage}}
  \caption{Benchmar k example task illustrating symmetry, difficulty scaling, and evaluation via I/O contracts with MCP 5D logging.}
  \label{fig:benchmark_example}
\end{figure}


==> figures/fig_failures.tex <==
\begin{figure}[t]
  \centering
  % Two side-by-side panels using minipage
  \begin{minipage}[t]{0.47\linewidth}
    \centering
    \begin{tikzpicture}[x=0.12cm,y=0.5cm]
      % Axes
      \draw[->] (0,0) -- (40,0) node[below] {ticks};
      \draw (0,-0.2) -- (0,1.8);
      \node[left] at (0,1) {lamp};
      % Desired waveform (green)
      \draw[thick,green!60!black] (2,0) -- (2,1) -- (14,1) -- (14,0);
      % Actual waveform (red) shifted by +2 ticks
      \draw[thick,red] (4,0) -- (4,1) -- (16,1) -- (16,0);
      % Tolerance window
      \draw[dashed,gray] (2, -0.2) -- (2, 1.6);
      \draw[dashed,gray] (3, -0.2) -- (3, 1.6);
      \node[gray] at (2.5,1.5) {$\pm1$ tick};
      % Violation mark
      \draw[<->,red] (3,1.3) -- node[above]{+2} (5,1.3);
      \node[anchor=west, font=\scriptsize] at (0,-0.8) {Desired (green) vs. actual (red) activation shows a +2 tick violation beyond $\pm1$ tolerance.};
    \end{tikzpicture}
    \vspace{0.2em}
    \caption*{(a) Timing violation (TE).}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.47\linewidth}
    \centering
    \begin{tikzpicture}[scale=0.9]
      % Blocks
      \node[draw,minimum width=1.2cm,minimum height=0.6cm,align=center] (btn) at (0,0) {Button};
      \draw (1.2,0) -- (3.0,0); % wire
      \node[draw,minimum width=1.4cm,minimum height=0.6cm,align=center] (rep) at (4.2,0) {Repeater};
      \node[draw,minimum width=1.2cm,minimum height=0.6cm,align=center] (lamp) at (6.2,0) {Lamp};
      % Correct orientation arrows
      \draw[->,green!60!black,thick] (3.0,0.3) -- (5.4,0.3) node[midway,above]{correct};
      % Incorrect orientation arrow (repeater facing left)
      \draw[->,red,thick] (5.4,-0.3) -- (3.0,-0.3) node[midway,below]{wrong};
      % X mark over repeater to indicate misalignment
      \draw[red,thick] (3.5,0.4) -- (4.9,-0.4);
      \draw[red,thick] (3.5,-0.4) -- (4.9,0.4);
      \node[anchor=west, font=\scriptsize] at (-0.2,-1.0) {Repeater facing away breaks power flow despite correct topology.};
    \end{tikzpicture}
    \vspace{0.2em}
    \caption*{(b) Orientation error (spatial).}
  \end{minipage}
  \caption{Representative failure cases. (a) Timing violation: output activation arrives +2 ticks outside the $\pm1$ tolerance window, counted in TE. (b) Orientation error: repeater direction mismatched to signal flow breaks propagation despite otherwise correct connectivity.}
  \label{fig:failures}
\end{figure}



==> tables/tab_ablation_guided_evolving.tex <==
\begin{table*}[!t]
 \centering
 \footnotesize

 \begin{tabular}{l c c}
 \toprule
 \textbf{Model} & \textbf{Method} & \textbf{Success $\uparrow$} \\
 \midrule
 \multirow{2}{*}{GPT-5} & No-guided evolving & 37 \\
 & Guided evolving & 68 \\
 \midrule
 \multirow{2}{*}{Claude 4.5} & No-guided evolving & 35 \\
 & Guided evolving & 65 \\
 \midrule
 \multirow{2}{*}{Qwen 3} & No-guided evolving & 20 \\
 & Guided evolving & 43 \\
 \midrule
 \multirow{2}{*}{Qwen2.5-72B-Instruct} & No-guided evolving & 14 \\
 & Guided evolving & 25 \\
 \midrule
 \multirow{2}{*}{Qwen3-32B} & No-guided evolving & 11 \\
 & Guided evolving & 19 \\
 \bottomrule
 \end{tabular}
 \vspace{-0.1in}
  \caption{Impact of guided evolution. With a simple directional hint (e.g., the keyword ``Signal-Flow-Direction''), performance nearly doubles. This suggests that correctly identifying the knowledge gap is the primary bottleneck, rather than the execution of experiments.}
 \label{tab:GuidedEvolution}
 \end{table*}

==> tables/tab_ablation_hint.tex <==
% Make sure you have these packages in your preamble:
% \usepackage{booktabs}

\begin{table}[h]
    \centering
    \footnotesize
    \begin{tabular}{l cc}
        \toprule
        \textbf{Model} & \textbf{Baseline w/ hint} & \textbf{Ours w/ hint} \\
        \midrule
        \texttt{gpt-5.2-2025-12-11} & -- & 37.0 $\rightarrow$ \textbf{67.5} \\
        \texttt{claude-opus-4-5-20251101} & -- & 35.0 $\rightarrow$ \textbf{65.0} \\
        \texttt{qwen3-235b-a22b-instruct-2507} & -- & 20.0 $\rightarrow$ \textbf{43.0} \\
        \texttt{qwen2.5-72b-instruct} & -- & 14.0 $\rightarrow$ \textbf{25.0} \\
        \texttt{qwen3-32b-instruct-2507} & -- & 10.5 $\rightarrow$ \textbf{19.0} \\
        \bottomrule
    \end{tabular}
    \caption{Guidance Ablation: Comparison showing the performance jump from our standard method to the guided version (w/ hint).}
    \label{tab:AblationHint}
\end{table}

==> tables/tab_ablation_with_knowledge_book.tex <==
\begin{table*}[!t]
  \centering
  \footnotesize
  \caption{Generalization of distilled knowledge across base LLMs under the S1 (reset) setting.
  The knowledge book, created through our self-evolving pipeline with one base model, is
  transferred to other LLMs without re-running the Scientist agent. This demonstrates that
  the distilled knowledge generalizes well across different model families and can improve
  performance even without model-specific self-evolution.
  All numbers are averaged over 8 runs.}
  \label{tab:KnowledgeTransfer}
  \begin{tabular}{l l r c c c}
  \toprule
  \textbf{Family} & \textbf{Model} & \textbf{Params} & \textbf{Open/Closed} &
  \textbf{Method} & \textbf{Acc $\uparrow$} \\
  \midrule
  \multirow{2}{*}{GPT family} & \multirow{2}{*}{GPT-5} &
  \multirow{2}{*}{--} & \multirow{2}{*}{Closed} & Direct LLM & 17.5 \\
   &  &  &  & LLM + Knowledge Book & 25.0 \\
  \midrule
  \multirow{2}{*}{Claude family} & \multirow{2}{*}{Claude 4.5} &
  \multirow{2}{*}{--} & \multirow{2}{*}{Closed} & Direct LLM & 16.5 \\
   &  &  &  & LLM + Knowledge Book & 23.5 \\
  \midrule
  \multirow{2}{*}{Qwen family} & \multirow{2}{*}{Qwen 3} &
  \multirow{2}{*}{1T MoE (32B)} & \multirow{2}{*}{Open} & Direct LLM & 9.5 \\
   &  &  &  & LLM + Knowledge Book & 14.0 \\
  \midrule
  \multirow{2}{*}{Qwen family} & \multirow{2}{*}{Qwen2.5-72B-Instruct} &
  \multirow{2}{*}{72B} & \multirow{2}{*}{Open} & Direct LLM & 6.5 \\
   &  &  &  & LLM + Knowledge Book & 10.0 \\
  \midrule
  \multirow{2}{*}{Qwen family} & \multirow{2}{*}{Qwen3-32B} &
  \multirow{2}{*}{32B} & \multirow{2}{*}{Open} & Direct LLM & 5.0 \\
   &  &  &  & LLM + Knowledge Book & 8.0 \\
  \bottomrule
  \end{tabular}
  \vspace{-0.1in}
  \end{table*}


==> tables/tab_knowledge_book_ablation.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l c}
    \toprule
    \textbf{Knowledge Consolidation Structure} & \textbf{w/Hint + Scientist} \\
    \midrule
    Self-determined Summary & $58.0$ \\
    \texttt{Finding-Explanation-Example} & $60.5$ \\
    \texttt{Claim-Proof-Constraints-Example} & $64.0$ \\
    \bottomrule
\end{tabular}
\caption{\textbf{Knowledge Consolidation Structure Ablation.} Success rates (\%) using Gemini-3-Pro with the scientist sub-agent and hints ($k/200 \times 100$, 8 runs). Vanilla knowledge consolidation via self-determined summaries reaches only 58.0\%---above using hints alone (see Gemini-3-Pro w/Hint in Table~\ref{tab:main_result_gap}). The structured \texttt{Claim-Proof-Constraints-Example} format performs best at 64.0\%.}
\label{tab:knowledge_consolidation_ablation}
\end{table}


==> tables/tab_llm_bases.tex <==
% % \begin{table*}[!t]
% %   \centering
% %   \footnotesize
% %   \caption{Performance across base LLMs under the S1 reset and S2 curriculum (L1--L5).
% %   Each base model is evaluated as a \textit{Baseline} agent (no Scientist,
% %   no knowledge book) and with our \textit{Ours} pipeline (Scientist
% %   experiments + Engineer reuse). Metrics: Acc (functional accuracy \%).
% %   All numbers are averaged over 8 runs.}
% %   \label{tab:LLMBases}
% %   \begin{tabular}{l l r c c c c}
% %   \toprule
% %   \textbf{Family} & \textbf{Model} & \textbf{Params} & \textbf{Open/Closed} &
% %   \textbf{Method} & \textbf{Acc S1 (reset) $\uparrow$} & \textbf{Acc S2 (curric.) $\uparrow$} \\
% %   \midrule
% %   \multirow{2}{*}{GPT family} & \multirow{2}{*}{GPT-5} &
% %   \multirow{2}{*}{--} & \multirow{2}{*}{Closed} & Baseline & 31.2 & 32.4 \\
% %    &  &  &  & Ours & 48.5 & 53.1 \\
% %   \midrule
% %   \multirow{2}{*}{Claude family} & \multirow{2}{*}{Claude 4.5} &
% %   \multirow{2}{*}{--} & \multirow{2}{*}{Closed} & Baseline & 30.6 & 31.3 \\
% %    &  &  &  & Ours & 45.2 & 50.7 \\
% %   \midrule
% %   \multirow{2}{*}{Qwen family} & \multirow{2}{*}{Qwen 3} &
% %   \multirow{2}{*}{235B MoE (22B)} & \multirow{2}{*}{Open} & Baseline & 26.4 & 27.1 \\
% %    &  &  &  & Ours & 42.3 & 45.6 \\
% %   \midrule
% %   \multirow{2}{*}{Qwen family} & \multirow{2}{*}{Qwen2.5-72B-Instruct} &
% %   \multirow{2}{*}{72B} & \multirow{2}{*}{Open} & Baseline & 16.8 & 17.5 \\
% %    &  &  &  & Ours & 22.1 & 24.3 \\
% %   \midrule
% %   \multirow{2}{*}{Qwen family} & \multirow{2}{*}{Qwen3-32B} &
% %   \multirow{2}{*}{32B} & \multirow{2}{*}{Open} & Baseline & 13.5 & 14.2 \\
% %    &  &  &  & Ours & 19.4 & 21.6 \\
% %   \bottomrule
% %   \end{tabular}
% %   \vspace{-0.1in}
% %   \end{table*}

\begin{table*}[!t]
  \centering
  \footnotesize

  \label{tab:LLMBases}
  \begin{tabular}{l l c c c c}
    \toprule
    \makecell[c]{\textbf{Model}} & \makecell[c]{\textbf{Params}} & \makecell[c]{\textbf{Open/Closed}} &
    \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Success $\uparrow$} \\ \textbf{Independent}} & \makecell[c]{\textbf{Success $\uparrow$} \\ \textbf{Curriculum}} \\
    \midrule
    \multirow{2}{*}{GPT-5} &
    \multirow{2}{*}{--} & \multirow{2}{*}{Closed} & Baseline & 27.1 & 33.5 \\
     &  &  & Ours & 35.2 & 46.8 \\
    \midrule
    \multirow{2}{*}{Claude 4.5} &
    \multirow{2}{*}{--} & \multirow{2}{*}{Closed} & Baseline & 26.6 & 32.8 \\
     &  &  & Ours & 33.5 & 44.1 \\
    \midrule
    \multirow{2}{*}{Qwen 3} &
    \multirow{2}{*}{\makecell[l]{235B \\ MoE(22B)}} & \multirow{2}{*}{Open} & Baseline & 23.0 & 28.5 \\
     &  &  & Ours & 30.2 & 39.7 \\
    \midrule
    \multirow{2}{*}{\makecell[l]{Qwen2.5-72B \\ -Instruct}} &
    \multirow{2}{*}{72B} & \multirow{2}{*}{Open} & Baseline & 14.6 & 18.8 \\
     &  &  & Ours & 16.5 & 21.1 \\
    \midrule
    \multirow{2}{*}{Qwen3-32B} &
    \multirow{2}{*}{32B} & \multirow{2}{*}{Open} & Baseline & 11.7 & 15.5 \\
     &  &  & Ours & 14.2 & 18.8 \\
    \bottomrule
  \end{tabular}
  \vspace{-0.1in}
\caption{Performance across base LLMs under the Independent Setting (each task in each level is addressed from fresh), and Curriculum Setting (the knowledge is accumulated as tackling the task from L1 to L5).
  Each base model is evaluated with the LLM baseline and with our \textit{Ours} pipeline (Scientist
  experiments + Engineer reuse) that allows the same max amount of construction trials.  The metric is measured by calculating the percentage of tasks being successfully handled.).
  All numbers are averaged over 8 runs.}
\end{table*}


==> tables/tab_main_results_cur_gap.tex <==
% \usepackage{colortbl}
\definecolor{lightgray}{gray}{0.9}

\begin{table*}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2pt}
    \renewcommand{\arraystretch}{1.2}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{l c >{\columncolor{lightgray}}c c >{\columncolor{lightgray}}c c >{\columncolor{lightgray}}c}
    \toprule
        \textbf{Model} & \textbf{Baseline} &
        \textbf{\shortstack{Know. Iden. Gap \\ ($\delta_{id}, r_{\delta_{id}}$)}} &
        \textbf{w/ Hint} &
        \textbf{\shortstack{Discovery Gap \\ ($\delta_{ds}, r_{\delta_{ds}}$)}} &
        \textbf{w/ Hint + Scientist} &
        \textbf{\shortstack{Residual (App Gap) \\ ($\delta_{app}, r_{\delta_{app}}$)}} \\
        \midrule
        \texttt{gemini-3-pro}         & $26.0$ & $\Delta 26.5$ ($1.02\times$) & $52.5$ & $\Delta 11.5$ ($0.44\times$) & $64.0$ & $\Delta 36.0$ ($1.38\times$) \\
        \texttt{gpt-5.2}               & $25.5$ & $\Delta 25.5$ ($1.00\times$) & $51.0$ & $\Delta 9.0$ ($0.35\times$) & $60.0$ & $\Delta 40.0$ ($1.57\times$) \\
        \texttt{claude-opus-4.5}       & $21.0$ & $\Delta 25.0$ ($1.19\times$) & $46.0$ & $\Delta 13.0$ ($0.62\times$) & $59.0$ & $\Delta 41.0$ ($1.95\times$) \\
        \texttt{glm-4.7}               & $23.0$ & $\Delta 22.5$ ($0.98\times$) & $45.5$ & $\Delta 7.5$ ($0.33\times$) & $53.0$ & $\Delta 47.0$ ($2.04\times$) \\
        \texttt{grok-4}                & $22.5$ & $\Delta 20.0$ ($0.89\times$) & $42.5$ & $\Delta 14.0$ ($0.62\times$) & $56.5$ & $\Delta 43.5$ ($1.93\times$) \\
        \texttt{qwen3-235b}            & $18.5$ & $\Delta 24.0$ ($1.30\times$) & $42.5$ & $\Delta 13.0$ ($0.70\times$) & $55.5$ & $\Delta 44.5$ ($2.41\times$) \\
        \texttt{qwen2.5-72b}           & $14.0$ & $\Delta 15.0$ ($1.07\times$) & $29.0$ & $\Delta 14.0$ ($1.00\times$) & $43.0$ & $\Delta 57.0$ ($4.07\times$) \\
        \texttt{qwen3-32b}             & $10.5$ & $\Delta 27.0$ ($2.57\times$) & $37.5$ & $\Delta 9.0$ ($0.86\times$) & $46.5$ & $\Delta 53.5$ ($5.10\times$) \\
        \bottomrule
    \end{tabular}
    }

    \caption{\textbf{Model Performance and Gap Decomposition (Curriculum Setting).} Success rates (\%) aggregated across all 25 tasks (5 families $\times$ 5 levels) over 8 independent runs (i.e., $k/200 \times 100$). Gray columns show the marginal performance gain ($\delta$) from each intervention and its ratio to the baseline ($r_{\delta}$). Absolute gaps ($\delta$) decompose the 100\% performance space; ratios ($r_{\delta}$) normalize for baseline differences but are subject to ceiling/floor effects.}
    \label{tab:main_result_gap}
\end{table*}


==> tables/tab_related_work_comparison.tex <==
\begin{table*}[t]
    \centering
    \small
    \renewcommand{\arraystretch}{1.15}
    \begin{threeparttable}

    \label{tab:related_work_comparison}

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l l cccc l}
    \toprule
    \textbf{Cat.} & \textbf{Benchmark} &
    \textbf{3D} & \textbf{Temporal} &
    \textbf{Functional} & \textbf{Limited Knowledge} &
    \textbf{Eval. Metric} \\
    \midrule
    \multirow{2}{*}{\textit{Dynamics Discovery}} &
    DiscoveryWorld~\cite{jansen2024discoveryworld} & \xmark & \xmark & \checkmark & \xmark & Task Success \\
    & GeneDisco~\cite{mehrjou2022genedisco}        & \xmark & \xmark & \checkmark & \xmark & Discovery \\
    \addlinespace[0.3em]
    
    \multirow{3}{*}{\textit{Phys.-Gr. Building}} &
    BuildArena~\cite{xia2025buildarena}    & \checkmark & \xmark & $\bigcirc$ & \xmark & Physics Valid \\
    & BesiegeField~\cite{zhang2024besiegefield} & \checkmark & \xmark & $\bigcirc$ & \xmark & Physics Valid \\
    \addlinespace[0.3em]
    
    \multirow{6}{*}{\textit{Minecraft Construction}} &
    MineDojo~\cite{fan2022minedojo}         & $\bigcirc$ & \xmark & \xmark & \xmark & Visual Similarity \\
    & Voyager~\cite{wang2023voyager}         & \xmark & $\bigcirc$ & \xmark & \xmark & Task Success \\
    & GITM~\cite{zhu2024gitm}                & \xmark & $\bigcirc$ & \xmark & \xmark & Task Success \\
    & Creative-Agents~\cite{cai2024creative} & $\bigcirc$ & \xmark & \xmark & \xmark & Creativity \\
    & MCU~\cite{zheng2025mcu}                & $\bigcirc$ & \xmark & \xmark & \xmark & Multi-Dim Score \\
    & TeamCraft~\cite{qian2024teamcraft}    & $\bigcirc$ & \xmark & $\bigcirc$ & \xmark & Task Success \\
    \addlinespace[0.3em]
    
    \multirow{1}{*}{\textit{Functional Discover \& Build}} &
    \textbf{Ours} & \checkmark & \checkmark & \checkmark & \checkmark & Function Success \\

    \addlinespace[0.3em]
    \bottomrule
    \end{tabular}%
    }
    
    \begin{tablenotes}[flushleft]
    \footnotesize
    \item \checkmark\ Full support;\quad $\bigcirc$\ Partial;\quad \xmark\ No support.
    \item \textbf{Limited Knowledge}: Tasks require domain-specific knowledge that
    pre-trained models do not possess.
    \end{tablenotes}
    \caption{\textbf{Comparison of our benchmark with existing benchmarks} for construction, 
    device creation, and embodied AI. Our benchmark uniquely combines 3D spatial
    reasoning, temporal precision, functional reasoning, and tasks requiring
    domain-specific knowledge, thereby necessiting developing AI agents to synthesize scientist-like discovery and engineer-like building ability together.}
    \end{threeparttable}
\end{table*}

==> tables/tab_task_level_breakdown.tex <==
\begin{table}[!t]
\centering
\footnotesize
\caption{Per-level performance breakdown using the best-performing model with self-evolution. Accuracy degrades with task complexity from L1 (primitives) to L5 (complex). We also report tokens per attempt and Engineer trials. All numbers are averaged over 8 runs.}
\label{tab:TaskLevelBreakdown}
\begin{tabular}{l c c c c}
\toprule
\textbf{Level} & \textbf{\# Tasks} & \textbf{Acc $\uparrow$} & \textbf{Tokens/Attempt $\downarrow$} & \textbf{Trials$_{Eng}$ $\downarrow$} \\
\midrule
L1 (Primitives) & 8 & 89.8 $\pm$ 2.5 & 1600 & 1.4 \\
L2 (Multi-output) & 7 & 73.8 $\pm$ 3.2 & 1850 & 1.7 \\
L3 (Intermediate) & 6 & 45.6 $\pm$ 4.1 & 2200 & 2.3 \\
L4 (Advanced) & 5 & 20.0 $\pm$ 5.2 & 2800 & 3.1 \\
L5 (Complex) & 5 & 5.0 $\pm$ 2.8 & 3500 & 4.2 \\
\midrule
\textbf{Aggregate (L1-L5)} & 31 & 46.8 $\pm$ 3.6 & 2380 & 2.5 \\
\bottomrule
\end{tabular}
\vspace{-0.15in}
\end{table}

